Needs-driven Heterogeneous Multi-Robot Cooperation in Rescue Missions

This paper focuses on the teaming aspects and the role of heterogeneity in a multi-robot system applied to robot-aided urban search and rescue (USAR) missions. We propose a needs-driven multi-robot cooperation mechanism represented through a Behavior Tree structure and evaluate the system's performance in terms of the group utility and energy cost to achieve the rescue mission in a limited time. From the theoretical analysis, we prove that the needs-driven cooperation in a heterogeneous robot system enables higher group utility than a homogeneous robot system. We also perform simulation experiments to verify the proposed needs-driven collaboration and show that the heterogeneous multi-robot cooperation can achieve better performance and increase system robustness by reducing uncertainty in task execution. Finally, we discuss the application to human-robot teaming.

==> bib_original.tex <==
\begin{thebibliography}{99}

\bibitem{1} Serena Chan. ``Complex Adaptive Systems.'' MIT ESD.83 Research Seminar in Engineering Systems October 31, 2001/November 6, 2001.
\bibitem{2} Levin SA. ``Ecosystems and the biosphere as complex adaptive systems.'' Ecosystems, 1(5):431-6. 1998.
\bibitem{3} Beni G., Wang, J. ``Swarm Intelligence in Cellular Robotic Systems.'' In Proc. NATO Advanced Workshop on Robots and Biological Systems, Tuscany, Italy, June 26-30 (1989).
\bibitem{4} L. E. Parker, Daniela Rus, and Gaurav Sukhatme. ``{Multiple Mobile Robot Systems}.'' Chapter 53 of Springer Handbook of Robotics, Second Edition, B. Siciliano and O. Khatib, editors, 2016, pp. 1362--1363.
\bibitem{6} A.I. Mourikis, S.I. ``Roumeliotis: Optimal sensor scheduling for resource-constrained localization of mobile robot formations.'' IEEE Trans. Robotics {\bf 22}(5), 917-931 (2006).
\bibitem{7} S. Kloder, S. Hutchinson. ``Path planning for permutation-invariant multirobot formations.'' IEEE Trans. Robotics {\bf 22}(4), 650-665 (2006).
\bibitem{8} C.W. Reynolds. ``Flocks, herds and schools: A distributed behavioral model.'' ACM SIGGRAPH Comput. Gr. {\bf 21}, 25–34 (1987).
\bibitem{9} M.J. Mataric. ``Designing emergent behaviors: From local interactions to collective intelligence,.'' Proc. 2nd Int. Conf. Simul. Adapt. Behav. (1992) pp. 432-441.
\bibitem{10} T. Balch, R. Arkin. ``Behavior-based formation control for multi-robot teams.'' IEEE Trans. Robotics Autom. {\bf 14}(6), 926-939 (1998).
\bibitem{11} Y. Cao, W. Yu, W. Ren, G. Chen. ``An overview of recent progress in the study of distributed multi- agent coordination.'' IEEE Trans. Ind. Inf. {\bf 9}(1), 427-438 (2012).
\bibitem{12} R.M. Murray. ``Recent research in cooperative control of multi-vehicle systems.'' J. Dyn. Syst. Meas. Control {\bf 129}(5), 571-583 (2007).
\bibitem{13} Santoro N. ``Design and analysis of distributed algorithms.'' John Wiley \& Sons; 2006 Nov 3.
\bibitem{14} Erciyes K. ``Distributed graph algorithms for computer networks.'' Springer Science \& Business Media; 2013 May 16.
\bibitem{15} George Coulouris, Jean Dollimore, Tim Kindberg, Gordon Blair. ``{Distributed Systems Concepts and Design}.'' Fifth Edition, 2012
\bibitem{16} Gerhard Weiss, {Multiagent System}, Second Edition, 2013.
\bibitem{17} Jeff S. Shamma. ``{Cooperative Control of Distributed Multi-Agent Systems}.'' 2007.
\bibitem{18} John H. Holland, {Daedalus}, Vol. 121, No. 1, A New Era in Computation (Winter, 1992), pp. 17-30.
\bibitem{19} H. Wang, A. Kolling, N. Brooks, S. Owens, S. Abedin, P. Scerri, P.-j. Lee, S.-Y. Chien, M. Lewis, and K. Sycara. ``Scalable target detection for large robot teams.'' In Proc. of the 6th international conference on Human-robot interaction. ACM, 2011, pp. 363–370.
\bibitem{20} S. Swaminathan, M. Phillips, and M. Likhachev. ``Planning for multi- agent teams with leader switching.'' In 2015 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2015, pp. 5403–5410.
\bibitem{21} G. Wagner and H. Choset. ``Subdimensional expansion for multirobot path planning.'' Artificial Intelligence, vol. 219, pp. 1–24, 2015.
\bibitem{22} W. Luo, N. Chakraborty, and K. Sycara. ``Distributed dynamic priority assignment and motion planning for multiple mobile robots with kin- odynamic constraints.'' In 2016 American Control Conference (ACC). IEEE, 2016, pp. 148–154.
\bibitem{23} V. R. Desaraju and J. P. How. ``Decentralized path planning for multi- agent teams with complex constraints.'' Autonomous Robots, vol. 32, no. 4, pp. 385–403, 2012.
\bibitem{24} R. Olfati-Saber. ``Flocking for multi-agent dynamic systems: Algorithms and theory.'' IEEE Transactions on automatic control, vol. 51, no. 3, pp. 401–420, 2006.
\bibitem{25} G. Antonelli, F. Arrichiello, and S. Chiaverini. ``Flocking for multi- robot systems via the null-space-based behavioral control.'' Swarm Intelligence, vol. 4, no. 1, pp. 37–56, 2010.
\bibitem{26} M. M. Zavlanos, A. Jadbabaie, and G. J. Pappas. ``Flocking while preserving network connectivity.'' In 2007 46th IEEE Conference on Decision and Control. IEEE, 2007, pp. 2919–2924.
\bibitem{27} X. Yan, J. Chen, and D. Sun. ``Multilevel-based topology design and shape control of robot swarms.'' Automatica, vol. 48, no. 12, pp. 3122– 3127, 2012.
\bibitem{28} C. Belta and V. Kumar. ``Abstraction and control for groups of robots.'' IEEE Transactions on Robotics, vol. 20, no. 5, pp. 865–875, 2004.
\bibitem{29} N. Ayanian and V. Kumar.  ``Abstractions and controllers for groups of robots in environments with obstacles.'' In 2010 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2010, pp. 3537–3542.
\bibitem{30} H Hamann, H Wörn. ``A framework of space–time continuous models for algorithm design in swarm robotics.'' Swarm Intelligence, December 2008, 2(4), pp 209–-239.
\bibitem{31} Martinoli, A. ``Swarm intelligence in autonomous collective robotics: from tools to the analysis and synthesis of distributed control strategies.'' Ph.D. thesis, Ecole Polytechnique Féderale de Lausanne, 1999.
\bibitem{32} H. Hamann. ``Swarm Robotics: A Formal Approach.'' Springer, New York, 2018.
\bibitem{33} Winfield, A. F. T., Sav, J., Fernández-Gago, M.-C., Dixon, C., \& Fisher, M. `` On formal specification of emergent behaviours in swarm robotic systems.'' International Journal of Advanced Robotic Systems, 2(4), 2005. pp. 363-–370.
\bibitem{34} Soysal, O., Sahin, E. ``A macroscopic model for self-organized aggregation in swarm robotic systems.'' In E. Sahin, W. M. Spears, \& A. F. Winfield (Eds.), Lecture notes in computer science: Vol. 4433. pp. 27-–42. 2005. Berlin: Springer.
\bibitem{35} Gazi, V., Passino, K. M. ``Stability analysis of swarms.'' IEEE Transactions on Automatic Control, 48(4), 692–697. 2003.
\bibitem{36} Feddema, J. T., Lewis, C., \& Schoenwald, D. A. ``Decentralized control of cooperative robotic vehicles: theory and application.'' IEEE Transactions on Robotics and Automation, 18(5), 852–864. 2002.
\bibitem{37} Maslow A.H. ``A Theory of Human Motivation.'' Psychological Review, 50(4), 370-396. 1943.
\bibitem{38} Savage EL, Schruben LW. ``Eliminating event cancellation in discrete event simulation.'' In Proc. of the 27th Conference on Winter simulation 1995 (pp. 744-750). IEEE Computer Society.

\bibitem{39} Dahl J, Chetlur M, Wilsey PA. ``Event list management in distributed simulation.'' In European Conference on Parallel Processing 2001 Aug 28 (pp. 466-475). Springer, Berlin, Heidelberg.

\bibitem{40} Henderson TR, Lacage M, Riley GF, Dowell C, Kopena J. ``Network simulations with the ns-3 simulator.'' SIGCOMM demonstration. 2008 Aug 17;14(14):527.

\bibitem{41} Michael Otte, Michael Kuhlman, and Donald Sofge. ``Auctions for Multi-Robot Task Allocation in Communication Limited Environments.'' Autonomous Robots. pp 1-38, 29 January, 2019.
\bibitem{42} R. G. Smith and R. Davis. ``Frameworks for co-operation in distributed problem solving.'' IEEE Transaction on System, Man and Cybernetics, vol. 11, no. 1, 1981.
\bibitem{43} Samir Aknine, Suzanne Pinson, Melvin F. Shakun. ``An Extended Multi-Agent Negotiation Protocol.'', Autonomous Agents and Multi-Agent Systems, Jan 2004, 8(1).
\bibitem{44} Danny Weyns, Nelis Boucke, Tom Holvoet and Bart Demarsin. ``DynCNET: A Protocol for Dynamic Task Assignment in Multiagent Systems.''  First International Conference on Self-Adaptive and Self-Organizing Systems (SASO 2007).

\bibitem{45} Yang GZ, Bellingham J, Dupont PE, Fischer P, Floridi L, Full R, Jacobstein N, Kumar V, McNutt M, Merrifield R, Nelson BJ. ``The grand challenges of Science Robotics. Science Robotics.`` Science Robotics, 2018 Jan 31;3(14):eaar7650.

\bibitem{46} Colledanchise M, Ögren P. ``Behavior trees in robotics and AI: an introduction.'' CRC Press. 2018.
\bibitem{47} Colledanchise M, Parasuraman RN, Ogren P. ``Learning of behavior trees for autonomous agents.'' IEEE Transactions on Games. 2018 Mar 19.

\bibitem{48} Valencia R, Andrade-Cetto J. ``Active pose SLAM.'' In Mapping, Planning and Exploration with Pose SLAM 2018 (pp. 89--108). Springer, Cham.
\bibitem{49} Ahrenholz J.`` Comparison of CORE network emulation platforms.'' In 2010 Military Communications (Milcom) Conference 2010 Oct 31 (pp. 166--171). IEEE.

\end{thebibliography}

==> bibliography_ordered.tex <==
\begin{thebibliography}{99}



@incollection{valencia2018active,
  title={Active pose SLAM},
  author={Valencia, Rafael and Andrade-Cetto, Juan},
  booktitle={Mapping, Planning and Exploration with Pose SLAM},
  pages={89--108},
  year={2018},
  publisher={Springer}
}









\iffalse
\bibitem{6} A.I. Mourikis, S.I. ``Roumeliotis: Optimal sensor scheduling for resource-constrained localization of mobile robot formations.'' IEEE Trans. Robotics {\bf 22}(5), 917-931 (2006).
\bibitem{13} Santoro N. ``Design and analysis of distributed algorithms.'' John Wiley \& Sons; 2006 Nov 3.
\bibitem{14} Erciyes K. ``Distributed graph algorithms for computer networks.'' Springer Science \& Business Media; 2013 May 16.
\bibitem{15} George Coulouris, Jean Dollimore, Tim Kindberg, Gordon Blair. ``{Distributed Systems Concepts and Design}.'' Fifth Edition, 2012
\bibitem{16} Gerhard Weiss, {Multiagent System}, Second Edition, 2013.
\bibitem{17} Jeff S. Shamma. ``{Cooperative Control of Distributed Multi-Agent Systems}.'' 2007.
\bibitem{18} John H. Holland, {Daedalus}, Vol. 121, No. 1, A New Era in Computation (Winter, 1992), pp. 17-30.
\bibitem{19} H. Wang, A. Kolling, N. Brooks, S. Owens, S. Abedin, P. Scerri, P.-j. Lee, S.-Y. Chien, M. Lewis, and K. Sycara. ``Scalable target detection for large robot teams.'' In Proc. of the 6th international conference on Human-robot interaction. ACM, 2011, pp. 363–370.
\bibitem{20} S. Swaminathan, M. Phillips, and M. Likhachev. ``Planning for multi- agent teams with leader switching.'' In 2015 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2015, pp. 5403–5410.
\bibitem{25} G. Antonelli, F. Arrichiello, and S. Chiaverini. ``Flocking for multi- robot systems via the null-space-based behavioral control.'' Swarm Intelligence, vol. 4, no. 1, pp. 37–56, 2010.
\bibitem{26} M. M. Zavlanos, A. Jadbabaie, and G. J. Pappas. ``Flocking while preserving network connectivity.'' In 2007 46th IEEE Conference on Decision and Control. IEEE, 2007, pp. 2919–2924.
\bibitem{28} C. Belta and V. Kumar. ``Abstraction and control for groups of robots.'' IEEE Transactions on Robotics, vol. 20, no. 5, pp. 865–875, 2004.
\bibitem{38} Savage EL, Schruben LW. ``Eliminating event cancellation in discrete event simulation.'' In Proc. of the 27th Conference on Winter simulation 1995 (pp. 744-750). IEEE Computer Society.
\bibitem{39} Dahl J, Chetlur M, Wilsey PA. ``Event list management in distributed simulation.'' In European Conference on Parallel Processing 2001 Aug 28 (pp. 466-475). Springer, Berlin, Heidelberg.
\fi

\end{thebibliography}
